Enhancing searches for resonances with machine learning and moment decomposition

A key challenge in searches for resonant new physics is that classifiers trained to enhance potential signals must not induce localized structures. Such structures could result in a false signal when the background is estimated from data using sideband methods. A variety of techniques have been developed to construct classifiers which are independent from the resonant feature (often a mass). Such strategies are sufficient to avoid localized structures, but are not necessary. We develop a new set of tools using a novel moment loss function (Moment Decomposition or MoDe) which relax the assumption of independence without creating structures in the background. By allowing classifiers to be more flexible, we enhance the sensitivity to new physics without compromising the fidelity of the background estimation.

==> algs.tex <==
%%%%%%%%%%%%%%%%%%%%%   Algorithms.   %%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Algorithms}
% \label{app:algo}
% \begin{algorithm}[H]
% \Input{$m$ : A sorted tensor of the controlled feature.\newline
% $F$ : A 2-D tensor of CDFs of predictions. Sorted in $m$.}
% \Output{$\Tilde{F}$ : A 2-D tensor of the $n$th order Legendre decomposition of $F$.}
% \tcp{Obtain coefficients for Legendre polynomial decomposition}
%   $c_0$, $c_1$ ,$c_2$  = LegendreDecomoposition($F,m$)\;
% \If{$c_\mathrm{max}$\textup{ is not None}}
% {$c_1 = c_\mathrm{max}\tanh\frac{c_1}{c_\mathrm{max}}$\;
% }
% \If{\textup{monotonic}}
% {
% $c_2 = c_1\tanh\frac{c_2}{c_1}$
% }
% $\Tilde{F} = c_0P_0 + c_1P_1 +c_2P_2$ \tcp*{where $P_i$ is the $i$th legendre polynomial}
% \Return{$\Tilde{F}$}
%  \caption{Response function fitting}
% \end{algorithm}
% \pagebreak
% \begin{algorithm}[H]
% \Input{$M$ : A tensor of the controlled feature.\newline
% $S$ : A tensor of predictions.\newline
% $n$ is the number of bins of $m$ to use and \var{steps} is  the number of integration segments.}
% %\Output{\var{loss} : A scalar representing the difference between the response and its desired shape.}
% \Fn{\Fforward{$M$, $S$,n, \var{steps}}}
%     {Sort $S$ and $M$ by $M$\;
%     % $\mathrm{indices\_m\_sorted} = \argsort{(m)}$\;
%     % $\hat{y} = \hat{y}[\mathrm{indices\_m\_sorted}]$\;
%     % $m = m[\mathrm{indices\_m\_sorted}]$\;
%     $S.\textup{reshape}(n,n_m)$ \tcp*{$n_m = \lfloor \frac{N}{n} \rfloor$ \# points in each $m$ bin}
%     $M.\textup{reshape}(n,n_m)$ \; 
%     % \tcp*{$N - n_m$ points are dropped}
%     $y = \textup{linspace(0,1,\var{steps})}$\;
%     \For{$s$ \textup{in} $0, ...,\var{steps} -1$}
%         { \For{\textup{$b$ in $0, ..., n - 1$}}
%             { $F[s,b] = \frac{1}{n_m}\sum_{i=0}^{n_m} \Theta(y[s]-S[b,i])$}
%         }
%     \var{loss} = $\sum_{s,b}(F[s,b]-\Tilde{F}[s,b])^2\cdot dy$ \tcp*{$dy = \frac{1}{\var{steps}}$}
%     \KwRet \var{loss}
%     }
% \Input{$M$ : A 2-D tensor of the controlled feature has the shape ($n$,$n_m$).\newline
% $S$ : A 2-D tensor of of predictions has the shape ($n$,$n_m$).}
% %\Output{$\nabla$\var{loss} : A tensor of gradients with respect to $\hat{y}$.}
% \Fn{\Fbackward{$M,S$}}
%     { Compute bin centers $\overline{m}$ and widths $\Delta m$\\
%     $y = S.\textup{reshape}(n_mn)$\;
%     \For{\textup{$s$ in $0, ..., n_m n - 1$}}
%     { \For{\textup{$b$ in $0, ..., n - 1$}}
%         { $\hat{F}[s,b] = \frac{1}{n_m}\sum_{i}^{n_m} \Theta(y[s]-S[b,i])$}
%         $\var{residual}[s,b] = F[s,b]-\textup{Fit}(\hat{F})[s,b]$ \;
%     }
%     \For{\textup{$s$ in $0, ..., n_m - 1$}}
%     {\For{\textup{$b$ in $0, ..., n - 1$}}
%         { $\nabla\var{loss} = \var{residual}[s+bn_m,b]$}}
%     \If{$\textup{\var{order}}>=1$}
%     {\For{\textup{$s$ in $0, ..., n_m - 1$}}
%     {\For{\textup{$b$ in $0, ..., n - 1$}}
%         { $\nabla\var{loss} = \nabla\var{loss} + \sum_{i=0}^n-\frac{1}{2}\Delta \overline{m}[b]\var{residual}[s+bn_m,i]$}}}
%     \If{$\textup{\var{order}}==2$}
%     {\For{\textup{$s$ in $0, ..., n_m - 1$}}
%     {\For{\textup{$b$ in $0, ..., n - 1$}}
%         { $\nabla\var{loss} = \nabla\var{loss} + \sum_{i=0}^n-\frac{3}{2}\Delta m[b] \overline{m}[b]\overline{m}[i]\var{residual}[s+bn_m,i]$}}}
%         \KwRet $-\frac{2}{n n_m}\nabla{loss}$
%   }
  
%  \caption{\textsc{MoDe} Loss}
% \end{algorithm}


==> tmp.tex <==

\subsection[Moment Decomposition (MoDe)]{Beyond decorrelation - Moment Decomposition (\textsc{MoDe})}
We will demonstrate a new method that achieves state-of-the-art decorrelation but also has the ability to weaken the uniformity constraint without compromising the fidelity of background estimation.
We use the fact that any reasonably well-behaved function can be accurately approximated using a finite sum of orthogonal polynomials (Legendre, Hermite, Chebyshev, etc.) We call this $n$th moment description of a function a \textit{Moment Decomposition} of order $n$, or \textsc{MoDe}[$n$]. In this paper, we shall use Legendre polynomials to find the moment decomposition of the response of the classifier.

\paragraph{Proposition:} The uniformity constraint (Eq. \ref{eqn:uniform}) can be written in terms of $F(s|M,Y)$, the conditional cumulative distribution function (CDF) of scores at $s$, as follows 
\begin{align}
    F(f(x)=s|M=m,Y=y) = F(f(x)=s|Y=y) \; \forall \; m \in M \; \text{and} \; \forall s \in \mathcal{S} 
\end{align}
for one or multiple values $y$. In practice, this constraint is only applied to backgrounds ($Y=0$.) 

For the purposes of our implementation we will think about the conditional CDF as the CDF in a given $m$ bin and use the more compact notation $F(f(x) = s| M=m, Y=y) \rightarrow F_m(s)$. 
The method can be generalized to unbinned implementations which could be explored in future work.


We can force the learned function to be simple by penalizing higher order contributions to its moment decomposition. This can be done by adding a regularization term to the loss $ \mathcal{L}[f] = L_{\mathrm{class}} + \lambda L_{\mathrm{\textsc{MoDe}}} $ where

\begin{equation}
\label{eqn:loss}
   L_{\mathrm{\textsc{MoDe}}}= \sum_m \int_0^1 |F_m(s) - \Tilde{F}_m(s)|^2 ds  
\end{equation}
where $\Tilde{F}_m(s)$ is the moment decomposition of $F_m(s)$ and has the form 
\[ \Tilde{F}_m(s) = \sum_{i=0}^n c^i(s) P^i_m
\]
where $P^i_m$ is the $i$th-order Legendre polynomial over $m$, $c^i(s)$ is the $i$th Legendre coefficient at score $s$ and is computed as follows
\[c^i(s) = \frac{2i+1}{2} \int_{-1}^1 F(m,s)P(m) dm \approx \frac{2i+1}{2} \sum_m F_m(s) P_m\Delta_m
\]
where $\Delta_m$ denotes the width of bin $m$.  Note that we assume $m$ values are normalized over the range $[-1,1]$.
Using the zeroth order decomposition of $F_m(s)$, $\Tilde{F}_m(s) = c^0(s)P^0_m = c^0(s)$, penalizes any higher-order deviations, forcing $F_m(s)$ to be flat.
The \textsc{MoDe} loss is optimal when the integrand in Eq. \ref{eqn:loss} vanishes for all values of $s$, that is, when $F_m(s) = \Tilde{F}_m(s)$,  or
\begin{equation}
    F(f(x) = s| M=m, Y=y) = c(f(x) = s| Y=y)
\end{equation}
which of course happens exactly when $M$ and $f(X)=s$ are independent random variables.

Similarly, a first order decomposition loosens the uniformity constraint and allows for some linear dependence on $M$. One can proceed to higher orders allowing for more complex response functions. Fig \ref{fig:orders} shows clearly how the CDF converges to the moment decomposition specified in training on a toy model.

The previous computations involving conditional CDFs can be simplified greatly because of the from chosen for $L_{\textsc{MoDe}}$ in \ref{eqn:loss}. First, we can approximate the CDFs empirically at batch level as 

\begin{equation}
\label{eqn:CDF}
   F_m(s) \approx \frac{1}{n_m}\sum_i^{n_m} \Theta(s-s_i) \delta(m-m_i) 
\end{equation}
where $i$ runs over the $n_m$ samples in the batch that fall in bin $m$. The implementation provided uses equal content bins to avoid bias in favor of bins with large populations. An alternative choice could be made here if the bins are chosen to have a fixed predetermined width \cite{Rogozhnikov:2014zea}. Either way, the derivatives will have the form
\begin{equation}
    \label{eqn:dfds}
    \frac{\partial F_m(s)}{\partial s_i} = -\frac{1}{n_{m}} \delta(s-s_i)\delta(m-m_i)
\end{equation}
The delta functions in $s$ kill the integral and we are left with a well-behaved function which we can be used to perform gradient descent. This is the biggest advantage we gain for using the form in \ref{eqn:loss} over other goodness of fit statistical tests. Note that computing $L_\mathrm{MoDe}$ with high precision is unnecessary since we primarily care about its gradients with respect to $s_i$. Gradients with respect to the moments are calculated in a similar fashion. For example
\begin{align}
    \frac{\partial F^0_m}{\partial s_i} & = - \frac{\Delta_{m_i}}{2n} \delta(s-s_i) \\
    \label{eqn:df1ds}
    \frac{\partial F^1_m}{\partial s_i} & = - \frac{3\Delta_{m_i}}{2n}\overline{M}_m\overline{M}_{m_i}\delta(s-s_i) 
\end{align}
where $\overline{M}_m$ here is taken to be the mean in bin $m$. Using Eq. \ref{eqn:dfds} - \ref{eqn:df1ds} we can write the gradient of the loss as
\begin{align}
    \frac{\partial L_{\textsc{MoDe[1]}}}{\partial s_i} & = -\frac{2}{N} \sum_m [F_m(s_i) - F_m^0(s_i)-F_m^1(s_i)]\big[\delta_{m,m_i}- \frac{\Delta_{m_i}}{2}  - \frac{3\Delta_{m_i}}{2}\overline{M}_m\overline{M}_{m_i}\delta(s-s_i)\big]
\end{align}

An extension to weighted samples naturally generalizes as follows
\begin{equation}
\label{eqn:loss_weighted}
   L_{\mathrm{\textsc{MoDe}}}= \sum_m \int_0^1 \omega_m(s)|F_m(s) - \Tilde{F}_m(s)|^2 ds  
\end{equation}
where $w_m(s)$ is a weight function which, thanks to the delta functions, reduces to a prefactor of the form $w_m(s_i)$ in the $\partial/\partial s_i$ gradient. %https://en.wikipedia.org/wiki/Anderson\%E2\%80\%93Darling_test
\textcolor{Maroon}{Should probably mention that this is somewhat similar to the Anderson-Darling test.}

